Calculation and selection of silicon to glass anodic bonding modes based on the criterion of minimum residual stress

The goal of this work is a scientifically justified choice of efficient technological parameters of anodic bonding of silicon to glass, ensuring a minimum level of residual stresses. The relevance of this dissertation is determined by the continuous efforts to reduce the negative effects of the joint use of dissimilar materials in electronic devices. Theoretical and practical results: the temperature dependence of the true values of the coefficient of thermal expansion of popular glass brands in the temperature range from minus 100 \deg C to 500 \deg C were obtained; the ratio of thicknesses of silicon and glass that minimizes residual stress on the silicon surface was calculated; the technique of minimizing the residual stresses in silicon anodically bonded to glass was developed. Results of this research are applicable to MEMS devices design and simulations. The first chapter provides the analysis of the current state of research in the field of anodic bonding technology application. The second chapter is devoted to the experimental study of temperature dependence of the linear thermal expansion coefficient of the glass. Thermomechanical properties and composition of the following glass brands: LK5, Schott Borofloat 33, Corning 7740, Hoya SD-2 were measured. The third chapter describes the existing models of estimating the residual stresses in the silicon-glass bonds. Two models based on a theory of strength of materials and the classical lamination theory with an additional temperature dependence of coefficients of thermal expansion are proposed for further use. Residual stresses in silicon-glass bonds are estimated with these models and data from the preceding chapter. The fourth chapter describes the experiments carried out to confirm claims from the previous chapters. The proposed technique of minimizing residual stresses is described as steps for a device designer.

==> common/documentpreload.tex <==
\listfiles
%%% Проверка используемого TeX-движка %%%
\RequirePackage{ifxetex, ifluatex}
\newif\ifxetexorluatex   % определяем новый условный оператор (http://tex.stackexchange.com/a/47579)
\ifxetex
    \xetexorluatextrue
\else
    \ifluatex
        \xetexorluatextrue
    \else
        \xetexorluatexfalse
    \fi
\fi
\RequirePackage{etoolbox}[2015/08/02]   %Для продвинутой проверки разных условий
\newif\ifpresentation          % Условие, проверяющее, что документ --- презентация


==> common/pdfaxsetup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Variables initiating  %%%
\newcounter{colourmode}
\newcounter{pdftype}
\newcounter{iccinsert}

%% Control of colour mode and pdf type
\setcounter{colourmode}{1}  % 0 --- undefined; 1 --- cmyk (always for pdf/x); 2 --- rgb
\setcounter{pdftype}{2}     % 0 --- undefined; 1 --- pdf/x; 2 --- pdf/a
\setcounter{iccinsert}{0}   % 0 --- don't upload icc cmyk inside pdf/x; 1 --- upload icc cmyk inside pdf/x;
\newcommand{\pdfapart}{1}        % PDF/A part
\newcommand{\pdfaconformance}{B} % PDF/A conformance
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifxetex
%%%%Needs to be compiled with commandline: "xelatex.exe -synctex=1 -interaction=nonstopmode -output-driver="xdvipdfmx -V 3 -z 0" --shell-escape %.tex" % as PDF 1.3 required by PDF/X
\else
    \ifluatex
        % http://tug.org/TUGboat/tb37-1/tb115hagen-pdf.pdf
        \ifnum\luatexversion>81
            \RequirePackage{luatex85}
        \else
        \fi
    \else
    \fi
    \ifnumequal{\value{pdftype}}{1}{
        \pdfobjcompresslevel=0%
        \pdfminorversion=3% Setting version of pdf % must be set 3 for PDF 1.3 required by PDF/X
    }{}
    \ifboolexpr{test {\ifnumequal{\value{pdftype}}{2}} and test {\ifdefstring{\pdfapart}{1}}}{
        \pdfobjcompresslevel=0%
        \pdfminorversion=4%
    }{}
    \pdfinclusioncopyfonts=1% If positive, this parameter forces pdfTEX to include fonts from a pdf file loaded with \pdfximage, even if those fonts are available on disk. Bigger files might be created, but included pdf files are sure to be embedded with the adequate fonts; indeed, the fonts on disk might be different from the embedded ones, and glyphs might be missing.
\fi
\PassOptionsToPackage{safe, warn}{textcomp}


==> common/setup.tex <==
%% Режим черновика
\makeatletter
\@ifundefined{c@draft}{
  \newcounter{draft}
  \setcounter{draft}{0}  % 0 --- чистовик (максимальное соблюдение ГОСТ)
                         % 1 --- черновик (отклонения от ГОСТ, но быстрая сборка итоговых PDF)
}{}
\makeatother

%% Использование в pdflatex шрифтов не по-умолчанию
\makeatletter
\@ifundefined{c@usealtfont}{
  \newcounter{usealtfont}
  \setcounter{usealtfont}{0}    % 0 --- шрифты на базе Computer Modern
                                % 2 --- использовать пакет XCharter, при наличии подходящей версии
}{}
\makeatother

%%% Предкомпиляция tikz рисунков для ускорения работы %%%
\makeatletter
\@ifundefined{c@imgprecompile}{
  \newcounter{imgprecompile}
  \setcounter{imgprecompile}{1}   % 0 --- без предкомпиляции;
                                  % 1 --- пользоваться предварительно скомпилированными pdf вместо генерации заново из tikz
}{}
\makeatother

